Neural Program Generation Modulo Static Analysis

State-of-the-art neural models of source code tend to be evaluated on the generation of individual expressions and lines of code, and commonly fail on long-horizon tasks such as the generation of entire method bodies. We propose to address this deficiency using weak supervision from a static program analyzer. Our neurosymbolic method allows a deep generative model to symbolically compute, using calls to a static-analysis tool, long-distance semantic relationships in the code that it has already generated. During training, the model observes these relationships and learns to generate programs conditioned on them. We apply our approach to the problem of generating entire Java methods given the remainder of the class that contains the method. Our experiments show that the approach substantially outperforms state-of-the-art transformers and a model that explicitly tries to learn program semantics on this task, both in terms of producing programs free of basic semantic errors and in terms of syntactically matching the ground truth.

==> AlternateIntro.tex <==
Neural networks have been applied successfully to many generative modeling tasks, from images with pixel-level detail
\cite{oord2016pixel} to strokes corresponding to crude sketches \cite{ha2017neural} to natural language \cite{vinyals2015show}. More recently, they have begun to be applied to
the generation of source code of programs~\cite{raychev2014code,YinN17,chen2018tree,bayou,ling2016latent,parisotto2016neuro,svyatkovskiy2020intellicode,gemmell2020relevance}. Such {\em neural program generators} are trained to recognize and reproduce patterns in large corpora of open-source code. They have many
potential applications in programming systems, including automatically testing programming
tools~\cite{holler2012fuzzing} and assisting humans as they solve programming tasks~\cite{hindle2012naturalness,raychev2014code}.

%The problem of learning deep generative models of {source code} from large open-source corpora has attracted much attention in the recent past. Solutions to the problem have natural applications in software engineering, for example, in systems for code completion. 

% Current approaches to the deep generation of source code can be divided into two categories. Those in the first category~\cite{raychev2014code,YinN17,chen2018tree} represent source code as sequences or syntax trees; a neural network that controls a generator of program syntax is then trained on these structures.
% The second category~\cite{bayou} consists of ``neurosymbolic'' approaches that start by using a neural model (from the first category above) to generate {\em sketches}, or syntactic abstractions, of programs. Symbolic program synthesis techniques are then used to generate concrete programs from these abstractions. 

A key limitation of these methods is that they treat source code as pure syntax, and do not account for semantic constraints that \emph{any reasonable program must satisfy}. In principle, a neural model could learn the semantics of programs from syntax, given enough data.
In practice, such learning is infeasible for complex, general-purpose programming languages. % at least for the amounts of data that are available in current-day open-source corpora.
Consequently, state-of-the-art neural models for code in real-world languages commonly generate programs with elementary semantic errors, such as uninitialized variables, type-incorrect expressions, and non-terminating loops.
It is possible to {\em reject} such incorrectly generated programs using downstream methods;
however, such rejection is often inefficient and diminishes the benefits of using a neural generator. 


\begin{wrapfigure}[11]{r}{0.42\columnwidth}
\vspace{-6mm}
\begin{lstlisting}
public class FileUtil{
  String err;
  public int read(File f){...}
  
  /* write lines to file */ 
  public void write(
    File f, String str){??}}
\end{lstlisting}
\reducevspacebetweenfigureandcaption
\caption{Code completion as conditional program generation. The ``...'' represents code elided for brevity.}\label{fig:completion}
\end{wrapfigure}


% \begin{figure}
% \begin{lstlisting}
% public class FileUtils{
%   String err;
%   public int read(File f){...}
  
%   /* write lines to file */ 
%   public void write(File f, String str){??}}
% \end{lstlisting}
% \vspace{-0.1in}
% \caption{Code completion as conditional program generation. The ``...'' represents code elided for brevity.}\label{fig:completion}
% \vspace{-0.2in}
% \end{figure}
In this paper, we offer a step toward overcoming this limitation, through a framework that allows the deep generation of source code {\em modulo language-level constraints}. The key insight of our approach is that the constraints
enforced by a programming language are known a priori.
Accordingly, they can be
incorporated into training, and our framework does so. 
Our main result is that this
approach has significant benefits: other models trained on syntactic representations of programs that unfailingly abide by a constraint still violate constraints upon deployment, whereas our method significantly outperforms these models on the task of generating programs that obey the constraints.

Concretely, we represent language-level constraints using {\em attribute grammars}~\cite{MST:Knuth68}, which are like context-free grammars, but allow rules to be conditioned on symbolic {\em attributes} computed from the context in which a rule is fired.
In the program-generation setting, the context is an incomplete program, and rules are fired to replace a nonterminal (a stand-in for unknown code) in this program.
The attributes are semantic information (for example, symbol tables) propagated top-down and left-to-right
%\twr{better than "bottom-up" would be "left-to-right"} 
through the context. 

% Chris note: I redid this paragraph to not use any formalism.  
% At each step during generation, our model of {\em neural attribute grammars} ({\nag}s) first constructs a vector of attributes $A$ from the surrounding context;
% it then uses a neural {\em controller}, representing a probability distribution $P(R \mid A)$ over rules $R$ of the grammar, to select the next rule to fire.
%\twr{Not sure why we say "for the most part".
%Are you allowing for the possibility that the corpus contains programs that do not compile?
%}
% To learn the controller, we start with a corpus of programs that obey the invariants we want enforced.
%Through static analysis of these programs, we build a 
%set of $(A_i, R_i)$ pairs that associate attributes $A_i$ for contexts arising during the top-down construction of these programs with the rules $R_i$ that were chosen in those contexts. The learning objective is to maximize the likelihood of this dataset.

At each step during generation, our model of {\em neural attribute grammars} ({\nag}s) first constructs a vector of attributes from the surrounding context;
it then uses a neural {\em controller} to compute a probability distribution over rules of the grammar, that governs the selection of rules to fire.
To learn the controller, we start with a corpus of programs that obey the invariants we want enforced.
Through static analysis of each program, we build a 
training set in which each data point associates the contexts arising during the top-down construction of a program with the attributes of the context and the rule that was chosen in that context.
% The learning objective is to maximize the likelihood of this dataset.

%We desire 
%the generated code to meet a predefined set of semantic properties (for example, type safety) and to also match the ground-truth code token by token. 

% Here, we are given a set of training pairs of the form (context, code to predict)
% \twr{This sentence about the training pairs we have contradicts the previous paragraph, which describes a different kind of training pair, namely (attribute values, rule choice).
% In fact, neither characterization is quite on target: each data point in the training set is really of the form (context, attribute values, rule choice).}
% where ``code to predict'' is a partial program that we want to predict (a missing method body in our Java evaluation) and ``context'' is the surrounding code (the class with the missing method body in our evaluation).  The goal is to use these pairs to learn a probability distribution over missing codes, given a partially completed Java class.  The goal at the heart of this paper is to ensure that the generated Java code is semantically correct: that typing and scoping rules are followed. We may want to ensure even more complex semantic properties, such as the correct usage of Java APIs.
% \textbf{Chris note: you took out the footnote, which I won't argue with, other than to say it happens to match really well with what Bishop says in the ML ``bible''.  Cut and pasted from Bishop: ``So far we have been quite careful to make a distinction between a random variable, such as the box $B$ in the fruit example, and the values that the random variable
% can take, for example $r$ if the box were the red one. Thus the probability that $B$ takes
% the value r is denoted $p(B = r)$. Although this helps to avoid ambiguity, it leads
% to a rather cumbersome notation, and in many cases there will be no need for such
% pedantry. Instead, we may simply write $p(B)$ to denote a distribution over the random variable $B$, or $p(r)$ to denote the distribution evaluated for the particular value
% $r$, provided that the interpretation is clear from the context.''  If you think it is obvious we can leave it out.}
% The objective is to use these pairs to learn a probability distribution $P(\Prog = \sProg \mid \sX, C(\sProg) = \textrm{true})$, over programs\footnote{In this paper, we adopt the convention of using a sans serif font $\sProg$ to denote a value, and an italic font $\Prog$ to denote a random variable. So, for example, $P(\Prog = \sProg)$ or simply $P(\sProg)$ refers to the value obtained by evaluating distribution function for random variable $\Prog$ at $\sProg$.}, that prioritizes programs that satisfy a semantic constraint $C$ and are relevant to a given label $\sX$.


We evaluate our approach in the \emph{conditional generation}~\cite{bayou} 
of Java methods 
over a large vocabulary of API methods and types.
Concretely, our goal is to generate a missing method body, given a class in which the method occurs. 
To perform this evaluation, we train a {\nag}, %incorporates an attribute grammar 
with attribution rules for ten different semantic conditions, on a
corpus of 1 million curated Java programs.
Our experiments show that the {\nag} reliably generates programs that satisfy the corresponding constraints, while syntactic neural models do not. Also, this reliability does not come at the cost of precision: {\nag}s generate programs that, with high probability, syntactically resemble the ground truth for the label in a generation task.
% Finally, we demonstrate the high computational cost of using a syntactic neural model and rejecting incorrect programs during generation. 

%models trained on syntactic representations of programs that unfailingly abide by a constraint still violate constraints upon deployment, and our 
%approach significantly outperforms these models at generating programs that obey requirements.
%show that our method is able to reliably generate programs that abide by these requirements, in contrast to a syntactic model that does not have access to the requirements during training. 
%
In summary, this paper makes three contributions:
\begin{itemize}
  \item
    We present {\em neural attribute grammars} ({\nag}s), framework for deep generation of source code that 
    incorporates program semantics into the learning process. 
    
  \item We instantiate the framework in a system for the conditional generation of API-heavy Java code snippets. 
 
  \item
%  \twr{Please restate this properly: We create 10 {\nag}s, one for each of 10 experiments; however, each \nag has the full set of 10 semantic conditions?}
  We show the benefits of {\nag}s using an evaluation involving eleven semantic conditions and a large corpus of open-source code.
\end{itemize}

% The rest of the paper is organized as follows.
% Sec.~\ref{sec:overview} presents an overview of our approach.
% Sec.~\ref{sec:attribute} gives necessary background on attribute grammars. Sec.~\ref{sec:neuralgrammar} introduces conditional neural grammars for program synthesis.
% Sec.~\ref{sec:neuralattrgrammar} describes our contribution: neural modeling using attributes, including our learning and inference methodology.
% Sec.~\ref{sec:eval} presents our experimental results.
% Sec.~\ref{sec:relwork} discusses related work.
% Sec.~\ref{sec:conc} concludes.








==> ConditionalNeuralGrammar.tex <==


We introduce the notion of a \emph{conditional neural grammar} (CNG), which is a stochastic CFG, and then extend CNGs to {\nag}s, which also incorporate attributes.
CNGs resemble other proposals for probabilistic grammars (such as classical stochastic grammars \cite{baker1979trainable,lari1990estimation} or more modern variants
\cite{kusner2017grammar}), but provide a more general framework, which we extend to {\nag}s in Sect.~\ref{sec:neuralattrgrammar}.
A CNG makes few assumptions other than (1) a leftmost derivation is carried out, and (2) the probability distribution governing the expansion of a symbol in the grammar takes into account the sequence of all expansions so far, as well as an input value $\sZ$ upon which all expansions are conditioned.
While we call this a ``neural'' grammar, the probability distribution used need not invoke a neural network, although that is what the implementation evaluated in Section \ref{sec:eval} does.

Consider a grammar consisting of productions of the form
\begin{equation} 
  \label{eqn:grammar}
  \S ~:~ seq_1 \textrm{ }|\textrm{ } seq_2 \textrm{ }|\textrm{ } seq_3... \textrm{ }|\textrm{ } seq_n
\end{equation} 
In a CNG, each symbol such as $\S$ corresponds to a categorical random variable with sample space $\Omega(\S) = \{seq_1, seq_2, ..., seq_n\}$. A trial over the symbol $\S$ randomly selects one of the RHS sequences for that symbol. If $\S$ is a terminal symbol, then $\Omega(\S) = \{\epsilon\}$, where $\epsilon$ is a special value that cannot be expanded. 
Subsequently, when a trial over $\S$ is performed and an RHS sequence from $\Omega(\S)$ is randomly selected, we will use the sans-serif $\sS$ to denote the identity of the RHS sequence observed.  

Now consider a depth-first, left-to-right algorithm for non-deterministically expanding rules in the grammar to generate a \emph{program} $\sProg = \langle (\S_1, \sS_1), (\S_2, \sS_2), ...\rangle$; here, each $\S_i$ is a symbol encountered during the expansion, and each $\sS_i$ is the identity of the RHS chosen for that symbol.

Let $\S_1$ correspond to the symbol $\id{Start}$.
We perform a trial over $\S_1$ and select one of the RHS sequences from $\Omega(\S_1)$. 
Let the identity of the RHS sequence selected be $\sS_1$.
Note that $\sS_1$ is \emph{itself} a sequence of symbols.  
Choose the first symbol in the sequence $\sS_1$; call this symbol $\S_2$.
Perform a trial over $\S_2$, and let the identity of the RHS sequence chosen be $\sS_2$.
Choose the first symbol in $\sS_2$ (call it $\S_3$) and expand it the same way.  This recursive descent continues until a terminal symbol $\S_i$ is encountered.  In this case, $\sS_i = \epsilon$, and the recursion unwinds.  If the recursion unwinds to symbol $\S_2$, for example, then we choose the second symbol in the sequence $\sS_1$, which we call $\S_{i + 1}$.  We perform a trial over $\S_{i + 1}$, and let the identity of the RHS sequence chosen be $\sS_{i + 1}$.  This sequence is then recursively expanded.  
Once all of the symbols in the RHS associated with the $\id{Start}$ symbol $\S_1$ have been fully expanded, we have generated a program.
The algorithm to generate a program using a CNG is given as Algorithm 1.  It is invoked with GenCNG$(\id{Start}, \langle \rangle, \sZ)$.


\begin{algorithm}[t]
\textbf{Input}: current symbol $\S$, sequence of symbols generated so far $\mathsf{SymSoFar}$, latent position $\sZ$ \smallskip \\
\textbf{Modifies}: all symbols expanded are appended to $\mathsf{SymSoFar}$
\eIf{$S \textrm{ is a terminal symbol}$}{
  Append $(\S, \epsilon)$ to $\mathsf{SymSoFar}$
}{
Choose a RHS sequence $\sS$ $\sim$ $P(\S | \mathsf{SymSoFar}, \sZ)$ \\
Append $(\S, \sS)$ to $\mathsf{SymSoFar}$ \\
\For{$\S' \in \sS \textrm{ in left-to-right order}$}{
        invoke GenCNG$(\S', \mathsf{SymSoFar}, \sZ)$
     }
}
\caption{GenCNG$(\S, \mathsf{SymSoFar}, \sZ)$}
\end{algorithm}


This algorithm defines a probability distribution $P (\Prog | \sZ)$, where for a particular program $\sProg$, the probability of observing $\sProg$ is computed as: 
\begin{align}
    P(\sProg | \sZ) = \prod_i & P(\S_i = \sS_i | \nonumber \\
    & \S_1 = \sS_1, ..., \S_{i - 1} = \sS_{i - 1}, \sZ). \nonumber
\end{align} 
We henceforth abbreviate the expression for the inner probability as $P(\sS_i | \sS_1, ..., \sS_{i - 1}, \sZ)$.
The CNG makes no assumption about the representation of this distribution;
typically, a sequential neural model of some sort (a recurrent neural network or a transformer) will be used to encode the sequence $\S_1 = \sS_1, ..., \S_{i - 1} = \sS_{i - 1}$.
Then, conditioned on $\sZ$, the sequence is decoded into a probability that $\S_i = \sS_i$. 


==> NeuralAttributeGrammars.tex <==

\subsection{Adding Attributes}

Now assume that the grammar of Eqn.\ (\ref{eqn:grammar}) is an $L$-attributed attribute grammar, so that each symbol $\S$ has an attribute set $A(\S)$. We use ${\uparrow}A(\S)$ to denote the synthesized attributes of $\S$, and ${\downarrow}A(\S)$ to denote the inherited attributes of $\S$.

% \footnote{In keeping with our notation where $\S$ corresponds to a symbol or random variable in the neural grammar and $\sS$ corresponds to a value taken by that variable in the derivation of a program, $A(\S)$ refers to the attributes associated with symbol $\S$, whereas $A(\sS)$ refers to the \emph{values} taken by those attributes during the derivation of a program.}

%Next, reconsider the sequence of symbols $\langle \x_1, \x_2, ..., \x_m \rangle$ corresponding to a program $\sProg$, generated via a depth-first non-deterministic expansion of the $\symb{Start}$ symbol.
%For symbol $\x_i$ in $\sProg$, let $\symb{Sibl}(\x_i)$ denote the set of values taken by symbols that are \emph{``older'' siblings} of $\x_i$ in $\sProg$.
%That is, reconsider the grammar of Equation \ref{eqn:grammar}.
%Assume that to generate $\x_i$ in $\sProg$, the symbol $\S_0$ was expanded to the sequence $\S_1^2 \textrm{ } \S_2^2 \textrm{ } \S_3^2 ... $, and $\x_i$ corresponds to value taken when $\S_4^2$ was expanded in the derivation of $\sProg$.
%Then $\symb{Sibl}(\x_i)$ is the list of values taken when $\S_1^2$, $\S_2^2$, and $\S_3^2$ were expanded in the derivation of $\sProg$.
%Note that this will be a triple $\langle \x_a, \x_b, \x_c \rangle$ where $a < b < c < i$, as symbols are always expanded left to right to form a program.
%Also, let $\symb{Par}(\x_i)$ refer to the value taken by the symbol that is a \emph{parent} of $\x_i$ in $\sProg$.
%In our example, this will be some $\x_d$ where $d < a < b < c < i$.
%Again, this is because of the depth-first expansion; the symbol $\S_0$ must be expanded before any of $\S_1^2$, $\S_2^2$, $\S_3^2$ or $\S_4^2$, and hence its corresponding value must be first in the sequence corresponding to $\sProg$.

A \nag corresponds to a CNG (as in Eqn.\  (\ref{eqn:cond})), where the conditional distribution $P(\Prog | \sZ)$ is defined as:
\begin{align}
P(\sProg | \sZ) = \prod_i P(\sS_i | \langle \sS_{1}, \sS_{2}, ..., \sS_{i-1} \rangle,
{\downarrow}A(\S_i), 
\sZ). \nonumber
\end{align}
\noindent
That is, when a symbol $S_i$ is non-deterministically expanded, its value depends not just on the latent position $\sZ$ and the sequence of expansions thus far, but also on the values of
$S_i$'s inherited attributes, ${\downarrow}A(\S_i)$.
In theory, a powerful enough learner with enough data could learn the importance of these sets of attribute values, without ever seeing them explicitly.
In that sense, they could be treated as latent variables to be learned. However, the benefit of having a compiler produce these values deterministically is that compiler authors know the semantic rules that must be followed by a program;
by presenting the data used to check whether those rules are followed directly to a learner, the process of learning to generate programs is made much easier.

Generation of a program under a \nag is described in Algorithm 2, where the distribution governing the expansion of symbol $S$ has access to attribute values ${\downarrow}A(S)$.


\begin{algorithm}[t]
\textbf{Input}: current symbol $\S$, inherited attrs ${\downarrow}A(S)$, sequence of symbols generated so far $\mathsf{SymSoFar}$, latent position $\sZ$ \\
\textbf{Modifies}: all symbols expanded are appended to $\mathsf{SymSoFar}$
\textbf{Returns}: ${\uparrow}A(S)$, the synthesized attributes of $S$ \\
\eIf{$S \textrm{ is a terminal symbol}$}{
  Append $(\S, \epsilon)$ to $\mathsf{SymSoFar}$ \\
  \Return $\emptyset$
}{
Choose an RHS sequence \\
$\textrm{  } \sS$ $\sim$ $P(\S | \mathsf{SymSoFar}, {\downarrow}A(S), \sZ)$ \\
Append $(\S, \sS)$ to $\mathsf{SymSoFar}$ \\
$\mathsf{SynthSoFar} \gets \langle \rangle$ \\
\For{$\S' \in \sS \textrm{ in left-to-right order }$}{
        Compute ${\downarrow}A(S')$ from ${\downarrow}A(S)$ and $\mathsf{SynthSoFar}$ \\
        ${\uparrow}A(S')$ $\leftarrow$ GenNAG$(\S', {\downarrow}A(S'), \mathsf{SymSoFar}, \sZ)$ \\
        Append ${\uparrow}A(S')$ to $\mathsf{SynthSoFar}$ 
     }
}
Compute ${\uparrow}A(S)$ from ${\downarrow}A(S)$ and $\mathsf{SynthSoFar}$ \\
\Return ${\uparrow}A(S)$
\caption{GenNAG$(\S, {\downarrow}A(S), \mathsf{SymSoFar}, \sZ)$}
\end{algorithm}


\subsection{Learning} \label{subsec:learning}

 We have access to a large corpus of training points, and wish to learn the parameters of $P(\Prog|\sX)$ via maximum likelihood.  Note that for a given $\sProg, \sX$ pair, 
\begin{align} 
P(\sProg|\sX) = &\int_\sZ P(\sZ|\sX) P(\sProg|\sZ) d\sZ \nonumber \\
= &\mathbb{E}_{\sZ \sim P(\sZ|\sX)}[P(\sProg|\sZ)] \nonumber
\end{align}
\noindent Because we learn via maximum likelihood, our goal, given a program $\sProg$, is to choose the the model parameters that maximize the value of $P(\sProg|\sX)$. Instead we may learn the same parameters by maximizing the logarithm of $P(\sProg|\sX)$. 
By Jensen's inequality, we know that
\begin{align} \label{eqn:training}
\log ( \mathbb{E}_{\sZ \sim P(\sZ|\sX)}&[P(\sProg|\sZ)] ) \nonumber \\
% &\le \mathbb{E}_{\sZ \sim P(\sZ|\sX)} [ \log P(\sProg|\sZ)] \nonumber \\
% &= \mathbb{E}_{\sZ \sim P(\sZ|\sX)} [ \log \prod_{\sS_i \in \sProg} P(\sS_i | ..., \sZ)] \nonumber \\
&\le \sum_{\sS_i \in \sProg} \mathbb{E}_{\sZ \sim P(\sZ|\sX)} [P(\sS_i | ..., \sZ)] \nonumber
\end{align}
Thus, given a training pair $\sProg, \sX$, we maximize the final summation, which serves as a lower bound to $P(\sProg|\sX)$, and is much easier to deal with.

To do this, given a large set of training examples of the form given in the equation as above, we use stochastic gradient ascent. For a particular training example, sample a vector $\mathsf{V}$ $\sim$ $\mathcal{N}(\vec{0}, \vec{1})$. Using the ``reparameterization trick'' \cite{kingma2013auto}, $\sZ = g(\mathsf{V})$ for some function $g$, which is itself a function of each of the various evidence encoders $f_1, f_2, ...$. Then, update the parameter set $\theta$ for the functions $f_1, f_2, ...$ and distribution function $P(\sS_i | ..., \sZ)$ in the direction $\nabla P(\sS_i | ..., g(\mathsf{V}))$.

\subsection{Designing a \nag}
\label{sec:DesigningANAG}

Intuitively, a \nag is likely to generate a semantically correct program because the presence of attributes provides key semantic clues.
In a conventional AG, productions are equipped with one or more attribute constraints to check whether key relationships hold among the values of the production’s attributes.
A \nag has no such constraints.
Our goal is to generate programs, and finding that a constraint is violated during generation requires a way to fix the violation---a problem we wish to avoid entirely.
We instead rely on a DNN to learn the appropriate relationships from training examples without constraint violations (e.g., the DNN finds that in the training data, the attribute values containing the formal and actual parameter types for a method call are always equal).
However, thinking of constraints provides a good mental model for designing an AG to be effective in a \nag.  That is, we generally want the attribute equations of the AG to be written so that if we did use constraints, the attributes necessary to check those constraints would be present where crucial choices will be made in the expansion---these sites are typically at the leaves of the grammar, where particular variables, types, and method calls are actually selected. 

An example of \nag design is in the supplementary material.



==> StaticAnalysisDesign.tex <==

Intuitively, a program generated with the aide of a static analyzer is likely to generate a semantically correct program because the static analysis provides key semantic clues during program generation.
In a conventional static analyzer, an AG would be used to maintain data structures that can be used to check, in an existing program, whether key relationships hold among the values of the production’s attributes.
Our goal is to generate and not validate programs.
However, thinking of constraints provides a good mental model for designing a static analysis that can provide a neural network with the clues necessary to generate a correct program.  That is, we generally want the attribute equations of the AG to be written so that if we did use constraints, the attributes necessary to check those constraints would be present where crucial choices will be made in the expansion---these sites are typically at the leaves of the grammar, where particular variables, types, and method calls are actually selected. 

An example of \nag design is in the supplementary material.

==> example_results/addItem_cng.tex <==
\begin{codefootnote}
void addItem(java.lang.Object fp_6){
  field_0.add((java.lang.Object) fp_1);
  return; }
\end{codefootnote}

==> example_results/addItem_nag.tex <==
\begin{codefootnote}
void addItem(java.lang.Object fp_6){
  field_1.add((java.lang.Object) fp_6);
  if (CONDITION){
    field_1.add((java.lang.Object) fp_6); }
  return; }
\end{codefootnote}


==> example_results/addItem_query.tex <==
\begin{codefootnote}
public class myClass{\
  String field_0; List<Object> field_1;
  
 /**add item to list if it does not exist*/
 @synthesize public 
  void addItem(Object fp_6){} }
\end{codefootnote}

==> example_results/addItem_transformer.tex <==
\begin{codefootnote}
public void additem ( object fp_6 ) { 
this . add ( fp_6 ) ) 
{ list . add ( fp_6 ) ; 
}

\end{codefootnote}

==> example_results/button_cng.tex <==
\begin{codefootnote}
JButton createButton() {
  javax.swing.JButton var_9;
  var_4.setToolTipText((String) ARG);
  var_4.addActionListener(
    (java.awt.event.ActionListener) ARG);
  return var_2; }
\end{codefootnote}


==> example_results/button_nag.tex <==
\begin{codefootnote}
JButton createButton () {
 javax.swing.ImageIcon var_3;
 javax.swing.JButton var_4;
 var_4 = new javax.swing.JButton.JButton(
 (java.lang.String) ARG,
  (javax.swing.Icon) var_3);
 var_4.addActionListener (
  (java.awt.event.ActionListener) ARG);
 var_4.addActionListener (
  (java.awt.event.ActionListener) ARG);
 return var_4; }
\end{codefootnote}


% \begin{codefootnote}
% javax.swing.JButton createButton(){
%   javax.swing.JButton var_8; 
%   var_8 = new javax.swing.JButton.JButton(
%     (String) ARG, (javax.swing.Icon) ARG);
%   var_8.setVerticalTextPosition((int) ARG);
%   var_8.setHorizontalTextPosition((int) ARG);
%   var_8.addActionListener((java.awt.event.ActionListener) ARG);
%   return var_8;
% }
% \end{codefootnote}

==> example_results/button_query.tex <==
\begin{codefootnote}
public class myGui{
public JFrame createFrame(final String title){
   JFrame frame = new JFrame(title);
   return frame;
}
/** create a button */
@synthesize public JButton createButton(){}}
\end{codefootnote}

==> example_results/button_transformer.tex <==
\begin{codefootnote}
public jbutton createbutton ( ) { 
     this . settitle ( ) ; 
     this . title ( ) ) ; 
     this . addactionlistener ) ; 
}
\end{codefootnote}

==> example_results/convert_cng.tex <==
\begin{codefootnote}
int convert(String fp_1){
  int var_2;
  Integer.parseInt((String) ARG);
  return var_3;
}
\end{codefootnote}


==> example_results/convert_nag.tex <==
\begin{codefootnote}
int convert(String fp_1){
  int var_8;
  var_8 = Integer.parseInt((String) fp_1);
  return var_8;
}
\end{codefootnote}


==> example_results/convert_query.tex <==
\begin{codefootnote}
public class myClass{
 /**
 */
  @synthesize public 
    int convert(String b){
  }
}
\end{codefootnote}


==> example_results/convert_transformer.tex <==
\begin{codefootnote}
public int convert ( string b ) 
{
 return b = = null ) 
 ? 0 : integer . parseint ( b ) ; 
}
\end{codefootnote}

==> example_results/reader_cng.tex <==
\begin{codefootnote}
String reader(){
  if (CONDITION){
   field_5.close(); }
  if (CONDITION){
   try {field_8 = field_4.readLine();
   } catch (java.io.IOException var_8) {
     var_0.printStackTrace(); }}
  return; }
\end{codefootnote}


==> example_results/reader_nag_2.tex <==
\begin{codefootnote}
java.lang.String reader(){
  java.lang.String var_2;
  try {
    field_3.readLine();
  }
  catch(java.io.IOException var_5){
    var_5.printStackTrace();
    if (CONDITION){
    try {
      var_5.close();
    }
    catch(java.io.IOException var_1){
       var_1.printStackTrace();
	}
   }
   return var_2;
 }
}
\end{codefootnote}

==> example_results/reader_transformer.tex <==
\begin{codefootnote}
public string reader ( ) {
  string reader = new String (
   reader reader.reader ( 
     new stringreader ) ; }
\end{codefootnote}
